Zero Bubble Pipeline Parallelism

Pipeline parallelism is one of the key components for large-scale distributed training, yet its efficiency suffers from pipeline bubbles which were deemed inevitable. In this work, we introduce a scheduling strategy that, to our knowledge, is the first to successfully achieve zero pipeline bubbles under synchronous training semantics. The key idea behind this improvement is to split the backward computation into two parts, one that computes gradient for the input and another that computes for the parameters. Based on this idea, we handcraft novel pipeline schedules that significantly outperform the baseline methods. We further develop an algorithm that automatically finds an optimal schedule based on specific model configuration and memory limit. Additionally, to truly achieve zero bubble, we introduce a novel technique to bypass synchronizations during the optimizer step. Experimental evaluations show that our method outperforms the 1F1B schedule up to 23% in throughput under a similar memory limit. This number can be further pushed to 31% when the memory constraint is relaxed. We believe our results mark a major step forward in harnessing the true potential of pipeline parallelism. We open sourced our implementation based on the popular Megatron-LM repository on https://github.com/sail-sg/zero-bubble-pipeline-parallelism.

==> background.tex <==
\section{Background}

Data, tensor, and pipeline parallelism are 3 main paradigms scaling the DL training.

\textbf{Data Parallelism (DP).} Dataset are sharded on multiple workers while model parameters are replicated among them. In the process of training iteration, gradients are aggregated and synchronized to produce new model parameters. Recent research on Data Parallelism focuses on decreasing memory footprint and reducing communication overheads for modern large models. Recompute strategy[ref] releases memory occupation of intermediate training results but incur duplicated computation. Mixed Precision Training[ref] encompasses lower precision numerical formats to achieve low memory usage and communication cost while trying to preserve accuracy. ZeRO[ref] can temporarily partition model parameters and optimizer states and gather them back once needed by introducing additional carefully designed communication. It also enables DP to shard on model parameters by only retaining a certain layer of the model at a time. Memory Offloading[ref] aims to exceed hardware limitations by incorporating CPU memory.

\textbf{Tensor Parallelism (TP).} Modern large models require being partitioned to scale beyond an individual server. Tensor Parallelism, sometimes referred as Model Parallelism or Operator Parallelism, divides a single tensor operator such as a matrix multiplication into multiple devices. Despite its tiny partition granularity, some operators, especially the widely used matrix multiplication, incur frequent reduction communication. This makes it suitable for multiple GPUs inside the same server with NVLink but generally not applicable between servers even with RDMA. Recent developments manage to come up with optimal tensor sharding policy to minimize communication cost by studying specific network architecture like Transformer[ref] or by proposing search-based optimizers given certain partition assumptions[ref].

\textbf{Pipeline Parallelism (PP).} As another paradigm on model sharding, Pipeline Parallelism instead partitions the entire model into a sequence of layers called stages and assigns them to each device. With the nature of intermediate granularity, communication mostly happens between stages for transporting activations, reaching lower communication compared to TP. However, each stage has to wait for the completion of its prior stage to get started, which massively hurts GPU utilization. Since its application, this idle time known as bubble has been the central bottleneck to be addressed.
Gpipe[ref] firstly breaks each mini-batch into many micro-batches to alleviate the dependence effect between adjacent stages. It relies on a large micro-batch number to reduce bubble rate to an ideal value. However, a large micro-batch number generally requires a large mini-batch, which enlarges memory footprint and slows down convergence[ref]. The improvements after it are mainly on the scheduling of micro-batches. Both 1F1B in PipeDream[ref] and Early Backward Scheduling in DAPPLE[ref] share a similar scheduling strategy to save memory by running backward as early as possible. Interleaved 1F1B[ref] further decreases bubble rate by increasing pipeline stages number without adding micro-batches at the cost of more communication. Chimera[ref] arranges micro-batches with different pipeline directions to better fill bubbles, but requires duplicating model parameters, which could be memory consuming when combined with optimizer states. There are also some asynchronous pipeline approaches that can dramatically increase utilization and save memory[ref][ref]. But they slow down convergence and model correctness so have not been practical.

Current state-of-the-art[ref] combines all these 3 parallelisms to adapt to the nature of hierarchical structure of hardware and achieves better performance. Hybriding them involves optimizing tensor sharding, device placement, and scheduling. Recent developments have proposed several handcrafted or search-based approaches trying to produce optimal decisions given certain partition assumptions.

==> introduction.tex <==
\section{Introduction}
As modern large Deep Neural Networks (DNN), especially Large Language Models(LLM), grow to billions of parameters[ref] and keep mounting, distributed training becomes essential to scale them beyond hardware limitations. Additionally, LLM training today may spend hundreds of thousands of GPU-days. Thus, distributed training also entails minimizing training time given restricted computation performance and memory in each accelerator such as GPU. However, prior attempts have shown a significant challenge on accelerators collaborating at scale with high utilization whilst reducing cost of inter-communication and redundant memory consumption. In particular, restricted mini-batch size has gradually been a critical hindrance to the further improvement in state-of-the-art solutions.

With current low-bandwidth interconnection between servers, adding accelerators typically requires more mini-batch data to increase computation-communication ratio for higher accelerator utilization. More importantly, both ZeRO based Data Parallelism and Pipeline Parallelism in current SOTA requires large batch sizes to scale out either data shards or pipeline micro-batches. However, large batch sizes do harm to model generalization and slow down the process of convergence, which makes training longer on the contrary. That leads us to the trade-off between reasonable batch sizes and accelerator utilization today.

While Data Parallelism seems to have intrinsic needs for large batch sizes as it shards on data, Pipeline Parallelism(PP) has potential solutions to ease this requirement. Traditional PP splits the entire model into a sequence of forward and backward layers across different devices. Each layer depends on the result of its last layer to start computation, leaving inevitable idle time referred to as the bubble. Previous work introduced further divided mini-batch called micro-batch to alleviate this dependence effect of PP from data perspective, where large batch sizes are needed to decrease the bubble ratio and improve utilization. From our point of view, even though dependency is impossible to be removed between adjacent layers, it is removable between operators inside each layer. By shifting layer-level to operator-level PP, it’s able to tackle the dependence effect from model perspective, making PP less rely on large batch sizes.

In this work, we present Zero-Bubble Pipeline Parallelism. Our key insight is once seeing stages in PP as smaller groups of operators instead of fixed layers, we have chances to completely squeeze bubbles away, resulting in smaller batch size compared to the previous approach. We also present a search algorithm for stage scheduling. Experimentally, our approach reaches up to 20\% faster than Megatron-LM while preserving the exact same training result.
